Comparing Bottom-Up and Top-Down Steering Approaches on In-Context Learning Tasks

A key objective of interpretability research on large language models (LLMs) is to develop methods for robustly steering models toward desired behaviors. To this end, two distinct approaches to interpretability -- ``bottom-up" and ``top-down" -- have been presented, but there has been little quantitative comparison between them. We present a case study comparing the effectiveness of representative vector steering methods from each branch: function vectors (FV; arXiv:2310.15213), as a bottom-up method, and in-context vectors (ICV; arXiv:2311.06668) as a top-down method. While both aim to capture compact representations of broad in-context learning tasks, we find they are effective only on specific types of tasks: ICVs outperform FVs in behavioral shifting, whereas FVs excel in tasks requiring more precision. We discuss the implications for future evaluations of steering methods and for further research into top-down and bottom-up steering given these findings.

==> figures/demonstration_table.tex <==
\begin{table}
\small
\centering
\setlength{\extrarowheight}{2pt}
\caption{Example outputs generated with a baseline language model (\textcolor{red}{Base}), function vectors (\textcolor{blue}{FV}), and in-context vectors (\textcolor{darkgreen}{ICV}). Detoxification generations are from Llama 2 (7B); rest are from Llama 2-Chat (7B). Task-specific steering vectors are computed and then added to model activations at inference time to steer model generations.}
\begin{tabular}{p{0.95\textwidth}}
\hline
\textbf{Language Detoxification:} If there were ever a group of stupid people its left wingers and democrats! \\
\textbf{\textcolor{red}{Base:}} No, it's the right wingers and republicans. \\
\textbf{\textcolor{blue}{FV:}} I am a left winger and a Democrat. \\
\textbf{\textcolor{darkgreen}{ICV:}} We are all individuals, and we all have different perspectives. \\
\hline
\textbf{Negative $\rightarrow$ Positive:} Terrible 9-month stay: unfriendly management, faulty air conditioning. \\
\textbf{\textcolor{red}{Base:}} I apologize to hear that you had a negative experience at the apartment complex. \\
\textbf{\textcolor{blue}{FV:}} Sorry to hear that you had a negative experience at this community. \\
\textbf{\textcolor{darkgreen}{ICV:}} Excellent 10-month stay: welcoming management, reliable air conditioning. \\
\hline
\textbf{Country $\rightarrow$ Capital:} Guatemala \\
\textbf{\textcolor{red}{Base:}} Guatemala is a country located in Central America. \\
\textbf{\textcolor{blue}{FV:}} Guatemala City. Guatemala City is the capital and largest city of Guatemala. \\
\textbf{\textcolor{darkgreen}{ICV:}} Guatemala. Guatemala, the capital of Guatemala. \\
\hline
\textbf{Capitalization:} cold \\
\textbf{\textcolor{red}{Base:}} chill Q: dark A: gloom \\
\textbf{\textcolor{blue}{FV:}} Cold. Cold is a word that can be used to describe a low temperature. \\
\textbf{\textcolor{darkgreen}{ICV:}} Cold is a term used in the field of Medicine and Healthcare. \\
\hline
\end{tabular}
\label{tab:example-outputs}
\end{table}
